AdaGNN: A multi-modal latent representation meta-learner for GNNs based on AdaBoosting

As a special field in deep learning, Graph Neural Networks (GNNs) focus on extracting intrinsic network features and have drawn unprecedented popularity in both academia and industry. Most of the state-of-the-art GNN models offer expressive, robust, scalable and inductive solutions empowering social network recommender systems with rich network features that are computationally difficult to leverage with graph traversal based methods. Most recent GNNs follow an encoder-decoder paradigm to encode high dimensional heterogeneous information from a subgraph onto one low dimensional embedding space. However, one single embedding space usually fails to capture all aspects of graph signals. In this work, we propose boosting-based meta learner for GNNs, which automatically learns multiple projections and the corresponding embedding spaces that captures different aspects of the graph signals. As a result, similarities between sub-graphs are quantified by embedding proximity on multiple embedding spaces. AdaGNN performs exceptionally well for applications with rich and diverse node neighborhood information. Moreover, AdaGNN is compatible with any inductive GNNs for both node-level and edge-level tasks.

==> deprecated/deprecated.tex <==
%Our goal is to upper bound the generalization error of $f\in\mathcal{C}$. For any  $g\in\mathcal{C}_K$ and $\theta>0$ in Lemma 3.7, we can write 
%\begin{equation*}
%\begin{split}
%&P_{\mathcal{D}}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0]\\
%&= P_{\mathcal{D}}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0,\ e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}] \\
%&\qquad+ P_{\mathcal{D}}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0,\ e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\geq\frac{\theta}{2}],\\
%&\leq P_{\mathcal{D}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]\\
%&\qquad + P_{\mathcal{D}}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0,\ e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\geq\frac{\theta}{2}],\\
%&\leq P_{\mathcal{D}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}] \\
%&\qquad + P_{\mathcal{D}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\geq\frac{\theta}{2}\ |\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0].
%\end{split}
%\end{equation*}

%Because this inequality is true for every $g(\mathcal{G}_i^L,\mathcal{G}_j^L)\in\mathcal{C}_K$, it's also true if we take an expectation of the RHS over any distribution we choose. Then we have
%\begin{equation*}
%\begin{split}
%&P_{\mathcal{D}}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0]\\
%&\qquad\leq \mathbb{E}_{g\sim\mathcal{Q}}[P_{\mathcal{D}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]] \\
%&\qquad + \mathbb{E}_{\mathcal{D}}[P_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\geq\frac{\theta}{2}\ |\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0]].
%\end{split}
%\end{equation*}

%\begin{align*}
%    \mathbb{E}_{g\sim\mathcal{Q}}[P_{\mathcal{D}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\geq\frac{\theta}{2}\ |\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0]]?
%\end{align*}


%a) Second term

%For the second term, we have $E_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))]=e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))$ since $E_{g\sim\mathcal{Q}}[g(\mathcal{G}_i^L,\mathcal{G}_j^L)]=f(\mathcal{G}_i^L,\mathcal{G}_j^L)$, then we could write the probability inside the expectation as
%\begin{equation*}
%\begin{split}
%&P_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\geq\frac{\theta}{2}\ |\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0]\\
%&\leq P_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))-\mathbb{E}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))]\geq\frac{\theta}{2}]\\
%&\leq P_{g\sim\mathcal{Q}}[|g(\mathcal{G}_i^L,\mathcal{G}_j^L)-\mathbb{E}[g(\mathcal{G}_i^L,\mathcal{G}_j^L)]|\geq\frac{\theta}{2}].   
%\end{split}
%\end{equation*}


%By Chernoff bound, we get
%$$
%P_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\geq\frac{\theta}{2}\ |\ e_{ij}(t-f\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0]\leq e^{-\frac{K\theta^2}{8}}.
%$$

%b) First term

%For any fixed $g\in\mathcal{C}_K$ and $\theta>0$, if we take a sample $S$ of size $m$, then consider the event in which the sample probability deviates from the true distribution by some value $\epsilon_K$, i.e. the event
%\begin{equation*}
%P_{\mathcal{D}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]>P_{\mathcal{S}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}] + \epsilon_K.
%\end{equation*}


%The probability of this event is at most $e^{-2m\epsilon_K^2}$ by Chernoff bound for any fixed $g$ and $\theta$ since the expected value of $P_{\mathcal{S}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]$ is $P_{\mathcal{D}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]$.

% Note that there are only $(K+1)$ possible choices for a nonnegative $\theta$ because $g(x_1,x_2)$ is a sum of $K$ values each of which is either $\pm1$. And there are only $|C_K|\leq |\mathcal{W}|^K$ possibilities for $g(x_1, x_2)$. So the union bound says the above event will occur with probability at most $(K+1)|\mathcal{W}|^Ke^{-2m\epsilon_K^2}$.

%For a bound over all $g$ and $\theta$, by Devroye, the above event will occur with probability at most $4e^8(K+1)(\frac{em^2}{d}^{dK})e^{-2m\epsilon_K^2}$.

%We could set $\epsilon_K=\sqrt{\frac{1}{2m}(dK\log(\frac{em^2}{d})+\log(\frac{4e^8(K+1)}{\delta_K}))}$ in order to make the probability of event is at most $\delta_K$.

%Since the bound holds in general, we could take the expectation with respect to $Q$. Then for any $\delta_K$, with probability at least $1-\delta_K$, we have 
%\begin{equation*}
%\begin{split}
%&P_{\mathcal{D},g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]\\
%&\qquad\qquad\leq P_{S,g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]+\epsilon_K. 
%\end{split}
%\end{equation*}




%On the other hand, we also have
%\begin{equation*}
%\begin{split}
%&P_{S,g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}] \\
%&= P_{S,g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2},\ e_{ij}(t-f(x_i,x_j))\leq\theta]\\
%&\qquad+ P_{S,g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2},\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))>\theta],\\
%&\leq P_{S}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\theta] \\
%&\qquad+ P_{S,g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}\ |\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))>\theta].
%\end{split}
%\end{equation*}




%Take the expectation of the second term in RHS, we could get
%\begin{equation*}
%\begin{split}
%&P_{S,g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}]\\
%&\leq P_{S}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\theta]\\
%&\qquad+ \mathbb{E}_S[P_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}\ |\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))>\theta]].
%\end{split}
%\end{equation*}



%Since $E_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))]=e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))$, by Chernoff bound,we have
%\begin{equation*}
%\begin{split}
%&P_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\frac{\theta}{2}\ |\ e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))>\theta]\\
%&\leq  P_{g\sim\mathcal{Q}}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))-\mathbb{E}[e_{ij}(t-g(\mathcal{G}_i^L,\mathcal{G}_j^L))]\leq -\frac{\theta}{2}]\\
%&\leq P_{g\sim\mathcal{Q}}[|g(\mathcal{G}_i^L,\mathcal{G}_j^L)-\mathbb{E}[g(\mathcal{G}_i^L,\mathcal{G}_j^L)]|\geq\frac{\theta}{2}]\\
%&\leq e^{-\frac{K\theta^2}{8}}.  
%\end{split}
%\end{equation*}




%By union bound, we set $\delta_K=\frac{\delta}{K(K+1)}$ in order to make the total failure probability be at most $\delta$. Then putting everything together, we would have
%\begin{equation*}
%\begin{split}
%&P_{\mathcal{D}}[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq0]\\
%&\leq P_S[e_{ij}(t-f(\mathcal{G}_i^L,\mathcal{G}_j^L))\leq\theta] + 2\exp(-\frac{K\theta^2}{8})\\
%&\qquad+\sqrt{\frac{1}{2m}(dK\log(\frac{em^2}{d})+\log(\frac{4e^8K(K+1)^2}{\delta}))}.    
%\end{split}
%\end{equation*}



%We could set $K=[(\frac{4}{\theta^2}\log\frac{m}{d})]$ to minimize the above bound since it's true for every $K$.





%\begin{theorem}
%The function $\phi$ computed by the GNN on the domain of graphs with up to $N$ nodes satisfies:
%\begin{itemize}
%    \item If $\sigma$ is Pfaffian with format ($\alpha,\beta,l$) then 
%    $$
%    \text{VCD}(\phi)\leq U(\alpha, \beta+1, lH, p,s, N);
%    $$
%    \item If $\sigma$ is the hyperbolic tangent function tanh or logistic sigmoid function logsig then 
%    $$
%    \text{VCD}(\phi)\leq U(2, 2, H, p,s, N);
%    $$
%    \item If $\sigma$ is an inverse tangent function atan then 
%    $$
%    \text{VCD}(\phi)\leq U(3, 2, 2H, p,s, N),
%    $$
%\end{itemize}
%where $U$ is defined as 
%\begin{equation*}
%\begin{split}
%U(\bar{\alpha},\bar{\beta}, \bar{l},\bar{p}, \bar{s}, \bar{N})&=M^2+2\bar{p}\log((\bar{\alpha}+2\bar{\beta}-1)(\bar{N}\bar{s}+1))\\
%&+2\log(2\bar{p}(\bar{\alpha}+\bar{\beta}-1)+2)+16\bar{p}+2,
%\end{split}
%\end{equation*}

%and $M=\bar{l}\bar{p}\bar{N}$.
%\end{theorem}

%\begin{theorem}
%If $\sigma$ is a piecewise polynomial of degree $d$ and $K$ pieces. Then, the function $\phi$ computed by the GNN on the domain of graphs with up to $N$ nodes satisfies
%$$
%\text{VCD}(\phi)=2(p-1)\log(2(d+1)(2d+1))+16p+2pR,
%$$
%where $p=3(s+L+1)H+s+1$ holds, and $R=\log(Ns+1)$ if $K=1$ and $R=\log((K^{NH}+2KNH)(Ns+1))$, otherwise.
%\end{theorem}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak



==> sections/definitions.tex <==
\paragraStartHighlight{Diffusion Induced Graph} A graph $\mathcal{G}^k = (\mathcal{V}, \mathcal{E}^k, \{w_{i,j}^k\in\mathbb{R}\})$ is a Diffusion Induced Graph (DIG) generated by latent affinities $\xi^k$ that flows on the whole graph, where $\mathcal{E}^k\in\mathcal{E}$ is the set of edges affected by $\xi^k$, $w^k_{i,j}\in[0,1]$ denotes the weight of $\xi^k$ and $\sum_{k=1}^Kw^k_{i,j}=y_{i,j}$. The same graph can have multiple DIGs with each representing a different "facet" of the same graph. \iffalse For example, some friendships are tighter than others on Facebook w.r.t. sports related topics whereas there might exist an orthogonal affinity mapping within political topics.\fi

\paragraStartHighlight{Node Entropy} We assign probability values to each node as $p(v_i)=\frac{\exp(-\Delta_i)}{\sum_{j=1}^{|\mathcal{V}|}\exp(-\Delta_j)}$, where $\Delta_i$ denotes the difference between node feature vector $x_i$ and its first order neighbors' node features, $\Delta_i=\sum_{k=1}^K\Delta_i^k=\sum_{k=1}^K\sum_{j\in\mathcal{N}_i\cap\mathcal{E}^k}w^k_{ij}(x_j-x_i)^T(x_j-x_i)$. Then we derive the node entropy as $H(v_i)=-p(v_i)\log p(v_i)$.


==> sections/entropy.tex <==
\begin{theorem}\label{def:entropy}
The sum of node entropy in Proposition 2 is lower than or equal to the node entropy in Proposition 1:
$$
\sum_{k=1}^{K}H^k(v_i)\leq H(v_i),
$$
when $\exp(1-\Delta_i^k)\leq\sum_{j=1}^{|\mathcal{V}|}\exp(-\Delta_j)$ for all nodes $v_i$.
\end{theorem}
\iffalse
\begin{proof}
By Jensen's inequality, nodes' probability values on diffusion induced network $\mathcal{G}^k$ are
$$
p^k(v_i)=\frac{\exp(-\Delta_i^k)}{\sum_{k=1}^K\sum_{j=1}^{|\mathcal{V}|}\exp(-\Delta_i^k)}\leq\frac{\exp(-\Delta_i^k)}{\sum_{j=1}^{|\mathcal{V}|}\exp(-\Delta_j)}=p^{k'}(v_i).
$$


Since $\Delta_i=\sum_{k=1}^K\Delta_i^k$, by Jensen's inequality, we obtain
$$
\sum_{k'}^{K=1}-p^{k'}(v_i)\log p^{k'}(v_i)\leq -p(v_i)\log p(v_i)= H(v_i).
$$

Since $\exp(1-\Delta_i^k)\leq\sum_{j=1}^{|\mathcal{V}|}\exp(-\Delta_j)$, which is easy to achieve when the number of training data is very large, we have $p^{k'}(v_i)\leq\frac{1}{e}$ and

$$
\sum_{k=1}^{K}H^k(v_i)=\sum_{k=1}^{K}-p^{k}(v_i)\log p^{k}(v_i)\leq\sum_{k'=1}^{K}-p^{k'}(v_i)\log p^{k'}(v_i),
$$
and then the sum of node entropy on diffusion induced network is lower than the whole graph:
$$
\sum_{k=1}^{K}H^k(v_i)\leq H(v_i).
$$
\end{proof}
\fi

Using Jensen's inequality, we can prove the above theorem. Proposition 2 lower the uncertainty while preserving the graph structure integrity. Moreover, it drops edges from the whole graph, increasing the effectiveness of GNNs in reducing over-smoothing and robustness during the whole training process.

==> sections/tables_backup.tex <==
\begin{table*}[h!]
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c|c| } 
\hline
&\multicolumn{4}{|c|}{Twitch} & \multicolumn{4}{|c|}{Linkedin} \\
\hline
Task & \multicolumn{2}{|c|}{Link Prediction (auc/ap)} & \multicolumn{2}{|c|}{Recommendation (ap)}& \multicolumn{2}{|c|}{Link Prediction (auc/ap)} & \multicolumn{2}{|c|}{Recommendation (ap)} \\
\hline
Problem&Transductive & Inductive & Transductive & Inductive&Transductive & Inductive & Transductive & Inductive\\
\hline
GAT-200             & 80.82/80.48 & 71.38/70.11 & 54.21 & 52.40 &&&&\\
GAT-1024            & 81.87/81.40 & 73.18/72.61 & 57.22 & 55.71 &&&&\\
GraphSage-3170      & 83.26/82.12 & 75.55/73.91 & 49.91 & 48.23 &&&&\\
GAT-3170            & 82.68/82.35 & 73.91/73.22 & 62.61 & 56.84 &&&&\\ 
\hline
AdaGraphSage-3170   & \textcolor{orange}{86.94/85.71} & \textcolor{orange}{79.18/77.49} & 53.40 & 51.60 &&&&\\
AdaGAT-200          & 82.53/81.75 & 73.09/71.27 & 57.10 & 54.71 &&&&\\ 
AdaGAT-1024         & 84.42/83.68 & 75.34/73.65 & 61.96 & 58.43 &&&&\\ 
AdaGAT-3170         & 86.10/85.30 & 77.60/75.71 & 71.64 & 64.37 &&&&\\ 
AdaGAT + Bootstrapping & 85.36/84.50 & 76.72/74.88 & 65.76 & 60.62 &&&&\\
AdaGAT-nn-200       & 85.27/84.59 & 75.05/73.33 & 91.33 & 68.40 &&&&\\ 
AdaGAT-nn-1024      & \textcolor{purple}{86.30/85.53} & \textcolor{purple}{76.70/75.13} & \textcolor{orange}{94.16} & \textcolor{orange}{70.52} &&&&\\
AdaGAT-nn-3170      & \textcolor{red}{87.51/86.78} & \textcolor{red}{79.25/77.73} & \textcolor{red}{94.79} & \textcolor{red}{73.40} &&&&\\
\hline
\end{tabular}
\end{center}
\caption{ROC AUC \% and Average Precision \% for multi-task learning, including link prediction and node recommendation, in transductive and inductive settings. \textcolor{red}{First}, \textcolor{orange}{Second}, \textcolor{purple}{Third} best performing method.}
\label{table:multi_task}
\end{table*}



\begin{table*}[h!]
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
&\multicolumn{2}{|c|}{Wikipedia}&\multicolumn{2}{|c|}{Movielens}&\multicolumn{1}{|c|}{Linkedin} \\
\hline
Task & \multicolumn{5}{|c|}{Link Prediction (auc)}  \\
\hline
Problem&Transductive & Inductive &Transductive & Inductive &Inductive  \\
\hline
\multicolumn{6}{|c|}{Static graph method}\\
\hline
GraphSage-1neighbor    & 92.50 & 93.42 & 56.94 & 55.65 &57.46\\
GAT               & 94.49 & 94.44 & 77.41 & 75.69 &65.08\\
\hline
AdaGraphSage-1neighbor & 94.86 & 95.62 & 63.20 & 62.15 &61.41\\
AdaGAT + Bootstrapping & 95.03 & 94.95 & 81.37 & 79.53 &\\
AdaGAT            & 95.09 & 95.02 & 79.40 & 77.50 &69.27\\
AdaGAT-nn         & \textcolor{purple}{96.20} & \textcolor{purple}{96.75} & \textcolor{red}{84.28} & \textcolor{red}{84.41}  &73.75\\
\hline
\multicolumn{6}{|c|}{Dynamic graph method}\\
\hline
% Jodie & ./94.62 & ./93.11 & ./. & ./. &\\
% TGAT  & ./95.34 & ./93.99 & ./. & ./. &\\
TGN & \textcolor{orange}{98.39} & \textcolor{orange}{97.77} & \textcolor{purple}{82.41} & \textcolor{purple}{81.48} &/ \\
\hline
AdaTGN& \textcolor{red}{98.91} & \textcolor{red}{98.32} & \textcolor{orange}{83.61} & \textcolor{orange}{82.47} & / \\
\hline
\end{tabular}
\end{center}
\caption{ROC AUC \% for future link prediction task in transductive and inductive settings. \textcolor{red}{First}, \textcolor{orange}{Second}, \textcolor{purple}{Third} best performing method.}
\label{table:temporal_graph}
\end{table*}

% \begin{table*}[h!]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
% &\multicolumn{2}{|c|}{Wikipedia}&\multicolumn{2}{|c|}{Movielens}&\multicolumn{1}{|c|}{Linkedin} \\
% \hline
% Task & \multicolumn{5}{|c|}{Link Prediction (auc/ap)}  \\
% \hline
% Problem&Transductive & Inductive &Transductive & Inductive &Inductive  \\
% \hline
% \multicolumn{6}{|c|}{Static graph method}\\
% \hline
% % GCN&&&&&&\\
% GraphSage-1neighbor    & 92.50/93.69 & 93.42/93.74 & 56.94/57.77 & 55.65/56.99 &57.46\\
% % GAT                    & 93.60/94.66 & 93.69/94.63 & 77.55/75.50 & 76.06/74.36 &65.08\\
% GAT               & 94.49/95.34 & 94.44/95.17 & 77.41/75.44 & 75.69/74.24 &65.08\\
% \hline
% % AdaGAT& 95.90 & 95.57 &&&&\\
% AdaGraphSage-1neighbor & 94.86/95.71 & 95.62/96.30 & 63.20/64.90 & 62.15/63.37 &61.41\\
% AdaGAT + Bootstrapping & 95.03/95.78 & 94.95/95.58 & 81.37/79.71 & 79.53/78.09 &\\
% % AdaGAT                 & 94.82/95.60 & 94.77/95.41 & 80.06/78.30 & 78.12/76.64 &69.27\\
% AdaGAT            & 95.09/95.83 & 95.02/95.65 & 79.40/77.71 & 77.50/76.10 &69.27\\
% % AdaGAT-nn              & 96.00/96.53 & 96.44/96.85 & \textcolor{orange}{84.09/82.62} & \textcolor{orange}{84.32/82.68} &73.75\\
% AdaGAT-nn         & \textcolor{purple}{96.20/96.70} & \textcolor{purple}{96.75/97.15} & \textcolor{red}{84.28/82.83} & \textcolor{red}{84.41/82.71}  &73.75\\
% \hline
% \multicolumn{6}{|c|}{Dynamic graph method}\\
% \hline
% % Jodie & ./94.62 & ./93.11 & ./. & ./. &\\
% % TGAT  & ./95.34 & ./93.99 & ./. & ./. &\\
% TGN & \textcolor{orange}{98.39/98.46} & \textcolor{orange}{97.77/97.81} & 82.41/80.94 & 81.48/79.96 &/ \\
% \hline
% AdaTGN& \textcolor{red}{98.91/99.00} & \textcolor{red}{98.32/98.40} & \textcolor{purple}{83.61/82.19} & \textcolor{purple}{82.47/81.03} & / \\
% \hline
% \end{tabular}
% \end{center}
% \caption{ROC AUC \% and Average Precision \% for future link prediction task in transductive and inductive settings. \textcolor{red}{First}, \textcolor{orange}{Second}, \textcolor{purple}{Third} best performing method.}
% \label{table:temporal_graph}
% \end{table*}
